Minimizing the AoI in Resource-Constrained Multi-Source Relaying Systems: Dynamic and Learning-based Scheduling

We consider a multi-source relaying system where independent sources randomly generate status update packets which are sent to the destination with the aid of a relay through unreliable links. We develop transmission scheduling policies to minimize the weighted sum average age of information (AoI) subject to transmission capacity and long-run average resource constraints. We formulate a stochastic control optimization problem and solve it using a constrained Markov decision process (CMDP) approach and a drift-plus-penalty method. The CMDP problem is solved by transforming it into an MDP problem using the Lagrangian relaxation method. We theoretically analyze the structure of optimal policies for the MDP problem and subsequently propose a structure-aware algorithm that returns a practical near-optimal policy. Using the drift-plus-penalty method, we devise a near-optimal low-complexity policy that performs the scheduling decisions dynamically. We also develop a model-free deep reinforcement learning policy for which the Lyapunov optimization theory and a dueling double deep Q-network are employed. The complexities of the proposed policies are analyzed. Simulation results are provided to assess the performance of our policies and validate the theoretical results. The results show up to 91% performance improvement compared to a baseline policy.

==> Figure/I-System_Model_and_Problem_Formulation.tex <==
\section{System Model and Formulation}
As shown in Fig. \ref{SM}, our considered system consists of a sensor (source), a monitor (destination), and a dual-band communication channel, i.e., channel between sensor-to-monitor and monitor-to-sensor\footnote{Commonly sensor-to-monitor channel is data channel and  monitor-to-sensor channel is feedback channel.}. 
\begin{figure}
    \centering
    \includegraphics{SystemModel.png}
    \caption{System model}
    \label{SM}
\end{figure}
We assume the continuous-time is slotted with the same and fixed slot time duration denoted by $\delta$. Each slot indexed by $t\in\Bbb{N}$. The sensor observes underlaying process which is modeled as discrete-time stochastic process as follows:
\begin{align}
\begin{split}
\label{Proc_Mod}
    &X(t+1)=f(X(t))+W(t),
%    \\&
 %   Y(t+1)=g(X(t))+V(t),
\end{split}
\end{align}
where $X(t)$ is the process and $W(t)$ is a stationary stochastic noise. $f(.)$ is an unknown function and can be a linear or non-linear function.
The model considered in \eqref{Proc_Mod} is more general and practical in comparison to linear model \cite{RE_twc}
%perfect observation \cite{LoosingInformation}
and can be applied for various systems and applications such as autonomous driving. The monitor has not direct access to the process and only has some samples of the process\footnote{Since each of two channels incurs a transmission delay, the sample's time on the monitor side is different from the reception time.}. 
%If these received sample are fresh, i.e., small time gaps between samples 
The monitor interest to fresh against to the process as possible. Let us, define that the monitor is at the maximum freshness, if it can reproduces the process $X(t)$. 
\\\indnet
Let $S_{i}(t)\in\{0,1\}$ be the sampling action, if $i$-th sample is generated and transmitted
%samples and transmits a  observed process
to the monitor at slot $t$, $S_i(t)=1$, otherwise $S_i(t)=0$. Notable $S(t)=0$ means the sensor is idle (or waiting) at slot $t$. Let $Y_{i}(t')$ denotes $i$-th received sample at slot $t'$ and is given by 
\begin{align}
    Y_i(t')=g(X(t))+V_i(t),~t'=t+D_i,
\end{align}
where $V_i(t)$ is a stationary stochastic noise which models the noise of channel and $D_i$ is discrete time variable captures the delay of channel \cite{Star2}. $g(X(t))=\mathds{1}_{\{S(t)=1\}}X(t)$, where $\mathds{1}_{\{\cdot\}}$ is the indicator function. As mentioned earlier, if the monitor can reproduce the process $X(t)$, meaning that all update information of the process in the sensor side is also available in the monitor side. 
%This is, the information of monitor about the undergoing process is freshest. If the monitor has all samples of the process for all times, meaning that similar to that the monitor observe the process. However, realization of this needs more sampling (sampling for all times), which is not resource efficient and infeasible for some setting \cite{}. Also, when the changing 
\\\indnet
Let $\bold{W}_{t}=\{(Y_{i}(t'),M): t'\le t\}$, indicates $M$ most recently samples that have been existed (both received and estimated) to the monitor until time $t$. By this, if a algorithm exits that uses these sample to estimate the next value of the process, i.e., $X(t+1)$ without getting its value from the sensor, we can say system is still fresh. 

%\\\indent
Let $\hat{X}(t)$ denotes the estimation of $X(t)$ at time $t$. This estimation is based on the samples of $Y_i(t)$, generally $\bold{W}_{t}$. 
Hence, we assume that $\hat{X}(t')=H(\bold{W}_{t}),t\le t'$, where $H(.)$ is a estimator function. Since in our model each transmitted sample experience a unknown random delay, it is impossible to have $\hat{X}(t')=X(t), \forall~ t'=t$, even the the value of $X(t)$ is transmitted, i.e., $S(t)=1$.
%Precisely, $H(.)$ is a estimator when 
One typical estimator design is based on the minimizing the  mean of square error defined as $(e(t))^2$, where $e(t)=\tilde{X}(t)-X(t)$. The minimum value of mean square errors implies that the monitor can accurately reproduce the process, hence the system is fresh. Estimation error commonly depends on the quality and quantity of available samples and the performance of the estimator. 
It is worthwhile to mention that we do not make any further assumptions about the  process model \eqref{Proc_Mod} as well as $V_i(t)$, e.g., Gaussian distribution. The main limitation of the mathematical solutions is considering some further assumptions on the model. This motivates us to (i) transform a general freshness management problem into a reinforcement learning framework and (ii) apply advance deep RL algorithm to handle the problem. We  discuss these in the following.  

\textcolor{blue}{Therefore, we intend to design a scheduling policy in order to minimizing the average estimation error under a maximum allowable sampling cost.
Formally, we interest in the following optimization problem:
\begin{align}
    \min_{\bold{S}} 
\end{align}
}
%To this end, the concept of age of these information is proposed in which with minimum AoI  
% \textcolor{orange}{ We consider two types of Markov sources, fast varying source (FVS) and slowly varying source (SVS) as depicted in Fig. \ref{}. Let $X_{i}(t),i\in\{1,2\}$ be the state, where $t\in\Bbb{N}$. Each state is represented by $M_i$ bits for each time instant $t$.
% We intend to provide optimal sampling policy in order to minimize  average age of information (AAoI) under minimum informative constraint. This constraint is defined in the following. 
% We assume the agent has no information about under laying process. We used information based data freshness metric \cite{YinSun}. From information theory, we have
% \begin{align}
%   & H(X_i(t))\le M_i\le H(X_i(t))+1,
%     \\
%   & H(X_i(t)|\bold{W}_i(t))\le M'_i\le H(X_i(t)|\bold{W}_i(t))+1,
% \end{align}
% where $M'_i$ is required bits \textcolor{blue}{differential coding} and  $\bold{W}_i(t)=\{(X_{i}(n),n):n\le t\},$ denote the samples that have been received by time $t$.  $n\in\mathcal{N}$ is the number of slot that the sampling action is performed presented  by $\mathcal{N}=\{n:\mathds{1}_{a_n}\}$. 
% \\\indent
% Our aim is to find an optimal policy to maximize long term mutual information defined by 
% \begin{equation}
% \limsup _{n \rightarrow \infty} \frac{1}{n} \mathrm{E}\left[\sum_{t=1}^{n} I(X_i(t),\bold{W}_i(t))\right].
% \end{equation}
% \textcolor{red}{How distinguish difference effects of successfully delivered and non delivered packets in the mutual information formula?}
% \textbf{Actions}
% \\
% \textbf{State}
% \\
% \textbf{Reward (discounted or averaged??)}
% \subsubsection{DRL Solution}
% }
